Code-less Patching for Heap Vulnerabilities Using Targeted Calling Context Encoding

Exploitation of heap vulnerabilities has been on the rise, leading to many devastating attacks. Conventional heap patch generation is a lengthy procedure, requiring intensive manual efforts. Worse, fresh patches tend to harm system dependability, hence deterring users from deploying them. We propose a heap patching system that simultaneously has the following prominent advantages: (1) generating patches without manual efforts; (2) installing patches without altering the code (so called code-less patching); (3) handling various heap vulnerability types; (4) imposing a very low overhead; and (5) no dependency on specific heap allocators. As a separate contribution, we propose targeted calling context encoding, which is a suite of algorithms for optimizing calling context encoding, an important technique with applications in many areas. The system properly combines heavyweight offline attack analysis with lightweight online defense generation, and provides a new countermeasure against heap attacks. The evaluation shows that the system is effective and efficient.

==> overview.tex <==
\section{Heaptherapy+ Overview}

\begin{figure}[ht]
    \centering
   \includegraphics[scale=.8]{images/mem-overview.pdf}
    
    \caption{The architecture of HeapTherapy+}
    \label{fig:overview}
\end{figure}

Figure \ref{fig:overview} shows the architectural overview of HeapTherapy+. There are three main components : i) A compiler pass for embedding calling context information in program binary, ii) A diagnosis module to detect memory vulnerability and generate patch file describing the protection needed for heap memory, iii) A shared library interposing the memory allocations and install patches to the vulnerable buffers. 
\par \textbf{Compilation:} As a first step of using Heaptherapy+, user have to compile the program with a calling context encoding instrumentation pass using LLVM compiler(\textit{clang}). We create a library (\textit{libPCC.so}) which will be used to instrument the user program with our instrumentation. Applying instrumentation pass during compilation is fairly easy. All the required by the user is to add some \textit{CFLAGS} during compilation: \textsf{"-Xclang  -load -Xclang libPCC.so"}.  
\par Additionally, the user program is also linked with the memory protection shared library(\textit{libheaptherapy}\textunderscore\textit{plus.so}).
As already mentioned, the memory protection shared library will protect the program's memory from attacks by interposing memory allocation and release functions. This compilation can easily adopted in any exiting program with almost no change in the previous configuration. The user only need to put the protection shared library into the programs library path and provide the following \textit{LDFLAGS} during compilation: "-ldl -lheaptherapy\textunderscore plus". 

\par \textbf{Diagnosis and Patch Generation:} The diagnosis and patch generation module will detect the vulnerabilities user program and generate the integer based patch file containing all the information needed to stop the memory corruption. This diagnosis will be performed in pre-deployment phase, and the whole diagnosis module will be executed offline. At this stage no heap protection is needed. Because to perform the diagnosis it is important to memory corruption is taken place. The user need to replace the shared library with a fake library with same name at this stage. The fake library is essentially a empty library, does nothing to protect the memory and only put into the place to avoid the linking error. \textit{LD}\textunderscore\textit{PROLOAD} option can also be used to achieve this context.

\par \textbf{Deployment:} At this stage the user program will be linked with the original memory protection shared library. The stared library will load the patch file generated by the diagnosis engine. By interposing all the memory allocations, it installs all the necessary patches to vulnerable user buffers ensuring no memory corruption occurs. Additionally the fast implementation of the shared library cause minimum overhead to the user program.
\\No code will be added or removed by Heaptherapy+. The user code will remain untouched throughout the process. Moreover, zero day vulnerability is also ensured.       

